A Systematic Approach to Computing the Manipulator Jacobian and Hessian using the Elementary Transform Sequence

The elementary transform sequence (ETS) provides a universal method of describing the kinematics of any serial-link manipulator. The ETS notation is intuitive and easy to understand, while avoiding the complexity and limitations of Denvit-Hartenberg frame assignment. In this paper, we describe a systematic method for computing the manipulator Jacobian and Hessian (differential kinematics) using the ETS notation. Differential kinematics have many applications including numerical inverse kinematics, resolved-rate motion control and manipulability motion control. Furthermore, we provide an open-source Python library which implements our algorithm and can be interfaced with any serial-link manipulator (available at github.com/petercorke/robotics-toolbox-python).

==> 3_dR.tex <==
\section{First Derivative of a Rotation} \label{sec:dR}

We refer the reader to Appendix \ref{sec:lie} for a background on rotations, Lie groups, Lie algebras, and \SO{3}. Derivatives of rotations are required when studying revolute joints. Consider a rotation in exponential form

\begin{equation*}
    \mat{R}(\theta(t)) = \textrm{e}^{ \skx{\evec{\omega}} \theta(t)} \in \SO{3}
\end{equation*}
%
where the rotation is described by the rotation axis $\evec{\omega}$, and a rotation angle $\theta(t)$. The time derivative of a rotation is given by the chain rule

\begin{align} \label{eq:dr0}
    \dfrac{d  \R(\theta(t))}
          {d t} =
    \dfrac{\partial \R(\theta)}
          {\partial \theta}
    \dfrac{\theta(t)}
          {d t}
\end{align}
%
where the partial derivative in (\ref{eq:dr0}) is 

\begin{align} \label{eq:dr1}
    \frac{\partial\mat{R}(\theta)}
         {\partial \theta} 
    &=
    \skx{\evec{\omega}} \ \textrm{e}^{\skx{\evec{\omega}} \theta(t)} \nonumber \\
    &= \skx{\evec{\omega}} \mat{R}(\theta(t)) 
\end{align}
%
to give the time derivative 

\begin{align} \label{eq:dr2}
    \dfrac{d  \R(\theta(t))}
          {d t}
    &=
    \skx{\evec{\omega}} \mat{R}(\theta(t)) \ \dot{\theta}
\end{align}
%
where $\vec{\omega} \in \mathbb{R}^3$ is the angular velocity and the following relationship holds

\begin{align*}
    \skx{\evec{\omega}} \dot{\theta} &= \skx{\vec{\omega}} \\
    \evec{\omega} \ \dot{\theta} &= \vec{\omega}
\end{align*}

The angular velocity describes the instantaneous rate of rotation about the x, y, and z-axis. The rotation axis $\evec{\omega}$, or angular velocity $\vec{\omega}$ can be recovered from (\ref{eq:dr1}) or (\ref{eq:dr2}) respectively, using the relationship in (\ref{eq:vex})

\begin{align} \label{m:dw}
    \evec{\omega} &= \iskx{ 
        \frac{\partial \matfn{R}{\theta(t)}}
             {\partial \theta}
    \matfn{R}{\theta(t)}^\mathrm{T} } \\
    \vec{\omega} &= \iskx{ 
        \frac{\mathrm{d} \matfn{R}{\theta(t)}}
             {\mathrm{d} t}
    \matfn{R}{\theta(t)}^\mathrm{T} }
\end{align}
%
since $ \mat{R} \in \SO{3}$, then $\mat{R}^{-1} = \mat{R}^\mathrm{T}$. 

Since we are concerned with rotations with an ETS, we only need to consider the elementary rotations $\mat{R}_x$, $\mat{R}_y$, and $\mat{R}_z$. Using the tangent space of \SO{3}, which is \so{3}, we can show that the partial derivative of each elementary rotation with respect to a rotation angle corresponds to one of the generators of \SO{3}

\begin{align*}
    \dfrac{\partial \mat{R}_x}
          {\partial \theta}
    &=     
    \begin{pmatrix}
        0 & 0 & 0 \\
        0 & 0 & -1 \\
        0 & 1 & 0 
    \end{pmatrix} \mat{R}_x(\theta), \\
    \dfrac{\partial \mat{R}_y}
          {\partial \theta}
    &=     
    \begin{pmatrix}
        0 & 0 & 1 \\
        0 & 0 & 0 \\
        -1 & 0 & 0 
    \end{pmatrix} \mat{R}_y(\theta), \\
    \dfrac{\partial \mat{R}_z}
          {\partial \theta}
    &=     
    \begin{pmatrix}
        0 & -1 & 0 \\
        1 & 0 & 0 \\
        0 & 0 & 0 
    \end{pmatrix} \mat{R}_z(\theta).
\end{align*}



\section{First Derivative of a Translation} \label{sec:ddT}

Taking the derivative of a pure translation follows a similar process to that of a pure rotation as in Section \ref{sec:dR}. We refer the reader to Appendix \ref{sec:lie2} for a background on homogeneous transformation matrices and \SE{3}. A derivative of a translation is required when considering a prismatic joint. By forming the translation into \SE{3} form, we obtain the time derivative as 

\begin{align} \label{eq:dt0}
    \dfrac{d  \T(\theta(t))}
          {d t} =
    \dfrac{\partial \T(\theta)}
          {\partial \theta}
    \dfrac{\theta(t)}
          {d t}
\end{align}

and since we are dealing with elementary translations the partial derivatives are simply obtained from the generators for \SE{3}

\begin{align*}
    \dfrac{\partial \mat{T}_x}
          {\partial \theta}
    &=     
    \begin{pmatrix}
        0 & 0 & 0 & 1 \\
        0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 
    \end{pmatrix} \mat{T}_x(\theta), \\
    \dfrac{\partial \mat{T}_y}
          {\partial \theta}
    &=     
    \begin{pmatrix}
        0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 1 \\
        0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 
    \end{pmatrix} \mat{T}_y(\theta), \\
    \dfrac{\partial \mat{T}_z}
          {\partial \theta}
    &=     
    \begin{pmatrix}
        0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 0 \\
        0 & 0 & 0 & 1 \\
        0 & 0 & 0 & 0 
    \end{pmatrix} \mat{T}_z(\theta).
\end{align*}

